Efficient Target Activity Detection based on Recurrent Neural Networks

This paper addresses the problem of Target Activity Detection (TAD) for binaural listening devices. TAD denotes the problem of robustly detecting the activity of a target speaker in a harsh acoustic environment, which comprises interfering speakers and noise (cocktail party scenario). In previous work, it has been shown that employing a Feed-forward Neural Network (FNN) for detecting the target speaker activity is a promising approach to combine the advantage of different TAD features (used as network inputs). In this contribution, we exploit a larger context window for TAD and compare the performance of FNNs and Recurrent Neural Networks (RNNs) with an explicit focus on small network topologies as desirable for embedded acoustic signal processing systems. More specifically, the investigations include a comparison between three different types of RNNs, namely plain RNNs, Long Short-Term Memories, and Gated Recurrent Units. The results indicate that all versions of RNNs outperform FNNs for the task of TAD.

==> abstract.tex <==
%
% SOF
%
\begin{abstract}
%
This paper addresses the problem of Target Activity Detection (TAD) for binaural listening devices.
TAD denotes the problem of robustly detecting the activity of a target speaker in a harsh acoustic environment, which comprises interfering speakers and noise (`cocktail party scenario').
In previous work, it has been shown that employing a Feed-forward Neural Network (FNN) for detecting the target speaker activity is a promising approach to combine the advantage of different TAD features (used as network inputs).
In this contribution, we exploit a larger context window for TAD and compare the performance of FNNs and Recurrent Neural Networks (RNNs) with an explicit focus on
small network topologies as desirable for embedded acoustic signal processing systems.
More specifically, the investigations include a comparison between three different types of RNNs, namely plain RNNs, Long Short-Term Memories, and Gated Recurrent Units.
The results indicate that all versions of RNNs outperform FNNs for the task of TAD.
%
%The work extends the classification scheme of Feed-forward Neural Networks (FNNs) to Recurrent Neural Networks (RNNs), in order to exploit the temporal evolution of the feature vectors.
%
\end{abstract}
%
% EOF
%

==> acronyms.tex <==

\begingroup     
\let\clearpage\relax        
\printglossary[type=\acronymtype]
\endgroup
	

==> acronymslist.tex <==
%
% SOF
%

% \newacronym{}{}{}


\newacronym{bte}{BTE}{Behind-the-Ear}

\newacronym{pc}{PC}{Personal Computer}
\newacronym{ram}{RAM}{Random-Access Memory}
\newacronym{os}{OS}{Operating System}
\newacronym{cpu}{CPU}{Central Processing Unit}
\newacronym{gpu}{GPU}{Graphics Processing Unit}
\newacronym{cudnn}{cuDNN}{NVIDIA CUDA Deep Neural Network library}
\newacronym{cuda}{CUDA}{Compute Unified Device Architecture}

\newacronym{numpy}{NumPy}{NUMerical PYthon}
\newacronym{scipy}{SciPy}{SCIentific PYthon}

\newacronym{tad}{TAD}{Target Activity Detection}
\newacronym{sinr}{SINR}{Signal-to-Interference-plus-Noise Ratio}
\newacronym{doa}{DOA}{Direction Of Arrival}
\newacronym{vad}{VAD}{Voice Activity Detection}

\newacronym{gru}{GRU}{Gated Recurrent Unit}

\newacronym{lstm2}{LSTM}{Long Short-Term Memory}
\newglossaryentry{lstm}
{
  name={LSTM},
  description={Long Short-Term Memory},
  first={\glsentrydesc{lstm} (\glsentrytext{lstm})},
  plural={LSTMs},
  descriptionplural={Long Short-Term Memories},
  firstplural={\glsentrydescplural{lstm} (\glsentryplural{lstm})}
}

\newacronym{cec}{CEC}{Constant Error Carousel}

\newacronym{ctc}{CTC}{Connectionist Temporal Classification}

\newacronym{rnn}{RNN}{Recurrent Neural Network}
\newacronym{fnn}{FNN}{Feed-forward Neural Network}
\newacronym{mlp}{MLP}{Multilayer Perceptron}

\newacronym{hsrnn}{HSRNN}{Hierarchical Subsampling Recurrent Neural Network}

\newacronym{bp}{BP}{Backpropagation}
\newacronym{bptt}{BPTT}{Backpropagation Through Time}
\newacronym{sgd}{SGD}{Stochastic Gradient Descent}

\newacronym{roc}{ROC}{Receiver Operator Characteristics}
\newacronym{auc}{AUC}{Area Under Curve}
\newacronym{mcc}{MCC}{Matthew's Correlation Coefficient}
\newacronym{acc}{ACC}{Accuracy}
\newacronym{tpr}{TPR}{True Positive Rate}
\newacronym{fpr}{FPR}{False Positive Rate}
\newacronym{tp}{TP}{True Positives}
\newacronym{tn}{TN}{True Negatives}
\newacronym{fp}{FP}{False Positives}
\newacronym{fn}{FN}{False Negatives}

\newacronym{pdf}{PDF}{Probability Density Function}

\newacronym{mse}{MSE}{Mean Square Error}
\newacronym{ace}{ACE}{Averaged Cross-Entropy}
\newacronym{ssd}{SSD}{Sum Squared Differences}

\newacronym{smote}{SMOTE}{Synthetic Minority Over-sampling Technique}

\newacronym{kemar}{KEMAR}{Knowles Electronics Manikin for Acoustic Research}
\newacronym{matlab}{MATLAB}{MATrix LABoratory}

\newacronym{srp}{SRP}{Steered Response Power}
\newacronym{msc}{MSC}{Magnitude Squared Coherence}
\newacronym{rtt}{RTT}{Relative Training Time}


%\newacronym{STFT}{STFT}{short-time Fourier transform}
%\newacronym{RIR}{RIR}{room impulse response}
%\newacronym{ASR}{ASR}{automatic speech recognition}
%\newacronym{DNN}{DNN}{deep neural network}
%\newacronym{WSJ}{WSJ}{wall street journal}
%
%\newglossaryentry{RIR}
%{
%  name={RIR},
%  description={room impulse response},
%  first={\glsentrydesc{RIR} (\glsentrytext{RIR})},
%  plural={RIRs},
%  descriptionplural={room impulse responses},
%  firstplural={\glsentrydesc{RIR}s (\glsentryplural{RIR})}
%}
%
%\newglossaryentry{WER}
%{
%  name={WER},
%  description={word error rate},
%  first={\glsentrydesc{WER} (\glsentrytext{WER})},
%  plural={WERs},
%  descriptionplural={word error rates},
%  firstplural={\glsentrydesc{WER}s (\glsentryplural{WER})}
%}


%
% EOF
%


==> keywords.tex <==

\begin{keywords}
	voice activity detection, target activity detection, recurrent neural networks, binaural listening devices
\end{keywords}

